Employing Social Media to Improve Mental Health Outcomes

As social media platforms are increasingly adopted, the data the data people leave behind is shining new light into our understanding of phenomena, ranging from socio-economic-political events to the spread of infectious diseases. This chapter presents research conducted in the past decade that has harnessed social media data in the service of mental health and well-being. The discussion is organized along three thrusts: a first that highlights how social media data has been utilized to detect and predict risk to varied mental health concerns; a second thrust that focuses on translation paradigms that can enable to use of such social media based algorithms in the real-world; and the final thrust that brings to the fore the ethical considerations and challenges that engender the conduct of this research as well as its translation. The chapter concludes by noting open questions and problems in this emergent area, emphasizing the need for deeper interdisciplinary collaborations and participatory research design, incorporating and centering on human agency, and attention to societal inequities and harms that may result from or be exacerbated in this line of computational social science research.

==> intervention.tex <==
\section{Social Media as an Intervention Platform}

In recent years, machine learning algorithms have begun to support tracking and intervention technologies in many health domains~\cite{}. However, most such tools enable only simplistic mechanisms to review one's data and require high compliance from individuals actively volunteering relevant information. These limitations prevent such tools from effectively supporting reflection, i.e., conscious re-examination of prior experiences to form new understanding. Reflection is a key to improved health and health maintenance, and recent work has shown the promise of data-driven health reflection. Effectively supporting reflection, however, requires more sophistication than simply showing a patient their data, especially in the context of mental health. Therefore, as a way to situate social media's potential in intervening for mental illness, we have focused on building tools to support reflection for eating disorders (ED) by combining voluntarily shared and unobtrusively gathered social media data with strategic presentation of machine learning analysis to cater to multi-stakeholder needs. To start with, we conducted interviews to understand the current practices of three stakeholders -- patients, clinicians, and support network members -- involved in ED reflection. Future research includes designing interactive tools that encapsulate these insights, alongside machine learning on patients' social media data, to support ED reflection. % among the three stakeholders. 
% The final phase will include evaluating these tools through a field deployment to understand how they become embedded in, and give rise to novel practices of ED reflection. 
We believe this research will result in novel mechanisms to support the treatment of devastating mental illnesses, going beyond existing personal  informatics tools by being sensitive to the complex psychological struggles of ED.


